Detecting Layout Templates in Complex Multiregion Files

Spreadsheets are among the most commonly used file formats for data management, distribution, and analysis. Their widespread employment makes it easy to gather large collections of data, but their flexible canvas-based structure makes automated analysis difficult without heavy preparation. One of the common problems that practitioners face is the presence of multiple, independent regions in a single spreadsheet, possibly separated by repeated empty cells. We define such files as "multiregion" files. In collections of various spreadsheets, we can observe that some share the same layout. We present the Mondrian approach to automatically identify layout templates across multiple files and systematically extract the corresponding regions. Our approach is composed of three phases: first, each file is rendered as an image and inspected for elements that could form regions; then, using a clustering algorithm, the identified elements are grouped to form regions; finally, every file layout is represented as a graph and compared with others to find layout templates. We compare our method to state-of-the-art table recognition algorithms on two corpora of real-world enterprise spreadsheets. Our approach shows the best performances in detecting reliable region boundaries within each file and can correctly identify recurring layouts across files.

==> acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acmart-master/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> experiments/old/1_dataset.tex <==
\subsection{Dataset analysis}
\label{subsec:evaluation-dataset}

The files in \DECO have been annotated with two levels of detail: cell-wise and range-wise.
A single \emph{cell} belongs to one of seven classes: \textsf{data}, \textsf{header}, \textsf{derived}, \textsf{group header}, \textsf{title}, \textsf{note}, and \textsf{other}.
A \emph{range} is a group of adjacent cells that are all labeled with one of the seven aforementioned labels.
A \textsf{table} is composed of one or more ranges, e.g., a data and a header range.
A detailed explanation of the labeling process can be found in~\cite{koci2019deco}.

To the extent that it is relevant to our work, we plan to detect the boundaries of all the different regions in a spreadsheet.
According to the annotation structure, these can be either tables or independent ranges, i.e., ranges that do not belong to any table.
In the following discussion, to avoid confusion, we use the term \emph{regions} to refer to the set composed of tables and independent ranges.
Whenever we refer to tables, we signify the subset of regions labeled as such.

% It is to consider that Excel allows users to hide rows or columns and merge together adjacent cells.
% This leads to inconsistencies between the actual content of a file and what a user can view or edit.
% Since the corpus has been annotated considering only visible information, to keep consistency in the csv files we omit the hidden fields altogether, and replicate the content of merged fields in all the cells that were merged together.

Table~\ref{tab:distribution-files} reports the distribution of files according to the categories defined in Section~\ref{subsec:taxonomy}: only around 27\% of the files belong to the single region class, of which 12.41\% show an apparently separated region.
The remaining 73\% spreadsheets, therefore, need data preparation in the form of \multifile~splitting.

\begin{table}[ht]
\centering
\def\arraystretch{1.2}
\begin{tabular}{rrr}
\multicolumn{1}{r|}{} & \multicolumn{1}{r|}{\# files} & \multicolumn{1}{r|}{\% files} \\ \hline
\multicolumn{1}{r|}{Single, non separated region} & \multicolumn{1}{r|}{127} & \multicolumn{1}{r|}{14.87\%} \\ \hline
\multicolumn{1}{r|}{Single, apparently separated region} & \multicolumn{1}{r|}{106} & \multicolumn{1}{r|}{12.41\%} \\ \hline
\multicolumn{1}{r|}{Multiple regions, single table} & \multicolumn{1}{r|}{450} & \multicolumn{1}{r|}{52.69\%} \\ \hline
\multicolumn{1}{r|}{Multiple regions, multiple tables} & \multicolumn{1}{r|}{171} & \multicolumn{1}{r|}{20.02\%} \\ \hline
\end{tabular}
\caption{Distribution of files per taxonomy of Section~\ref{subsec:taxonomy}}
\label{tab:distribution-files}
\end{table}

Table~\ref{tab:average-regions} reports on the average number and type of regions found in files, with a focus on table regions.
For spreadsheets containing only one region, this is necessarily a table.
However, files with only one table region show, on average, 2.79 regions.
For example, a spreadsheet may contain a table, a title, and a note region as metadata for the content of the table.
The number of regions naturally increases when considering files that contain multiple tables.
It is noteworthy that, considering multiple region files, the average number of regions corresponds closely to the product of their average number of tables and the average number of regions found in single table files (5.72 compared to $5.64 = 2.02 \times 2.79$).
The same behavior can be observed for the average number of regions in files that contain multiple tables: this can be estimated by multiplying their average number of tables times the average number of regions per single table files (10.99 compared to $13.11 = 4.7 \times 2.79$).
This behavior can be explained with the fact that having multiple tables often comes with having additional table metadata regions, as well as some global metadata such as spreadsheet titles or notes needed to interpret the different tables.

\begin{table}[ht]
\centering\small
\def\arraystretch{1.2}
\begin{tabular}{rrrrr}
\multicolumn{1}{r|}{} & \multicolumn{1}{r|}{\#files} & \multicolumn{1}{r|}{\%files} & \multicolumn{1}{r|}{\begin{tabular}[c]{@{}r@{}}Average \\ \# regions\end{tabular}} & \multicolumn{1}{r|}{\begin{tabular}[c]{@{}r@{}}Average \\ \# tables\end{tabular}} \\ \hline
\multicolumn{1}{l|}{Single region} & \multicolumn{1}{r|}{233} & \multicolumn{1}{r|}{27.28\%} & \multicolumn{1}{r|}{1.00} & \multicolumn{1}{r|}{1.00} \\ \hline
\multicolumn{1}{l|}{Multiple regions} & \multicolumn{1}{r|}{621} & \multicolumn{1}{r|}{72.72\%} & \multicolumn{1}{r|}{5.72} & \multicolumn{1}{r|}{2.02} \\ \hline
\multicolumn{1}{l|}{Single table} & \multicolumn{1}{r|}{683} & \multicolumn{1}{r|}{79.98\%} & \multicolumn{1}{r|}{2.79} & \multicolumn{1}{r|}{1.00} \\ \hline
\multicolumn{1}{l|}{Multiple tables} & \multicolumn{1}{r|}{171} & \multicolumn{1}{r|}{20.02\%} & \multicolumn{1}{r|}{10.99} & \multicolumn{1}{r|}{4.70} \\ \hline
\textbf{Total files} & \textbf{854} & \textbf{100.00\%} & \textbf{4.43} & \textbf{1.74}
\end{tabular}
\caption{Average number of regions/tables per class of files}
\label{tab:average-regions}
\end{table}

Figure~\ref{fig:histogram_regions} shows both the histogram and the cumulative percentage of the number of regions per file.
It can be noted that the distribution is skewed towards small values, with almost 95\% of the files having less than 10 regions.
The tail is however quite long -- one file has 321 regions. 
For the rest of the experiments, we consider outliers and therefore exclude the files with a number of regions greater than 99.9\% of the remaining files. 
\begin{figure}[ht!]
    \centering
    \includegraphics[width=\columnwidth]{figure/chap5/exp1/histogram_regions.png}
    \caption{Distribution of the number of regions per file}
    \label{fig:histogram_regions}
\end{figure}


With the cell-level annotations that accompany the \DECO dataset, we were able to also analyze, for a given region, its element composition.
Following the definitions given in Section~\ref{subsec:taxonomy}, Table~\ref{tab:connectivity} shows the type of connections between pairs of elements (belonging to the same region) and pairs of regions.
It can be seen that, in the regions that are composed of more than one element, those are separated.
If paired with the results showcased in Table~\ref{tab:distribution-files}, these numbers prove the inadequacy of a naive connected component recognition to find independent regions: even if multiple regions are mostly visually separated from each other, it would be impossible to distinguish separated elements belonging together.
Moreover, a non-negligible fraction (almost 4\%) of region pairs are intersecting.
\begin{table}[t]
\def\arraystretch{1.2}
\begin{tabular}{r|r|r|r|r|}
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Type of\\connection\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Inside \\one region\end{tabular}} & \multicolumn{1}{c|}{\%} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Across\\ regions\end{tabular}} & \multicolumn{1}{c|}{\%} \\ \hline
Separated & 221,215 & 97.89\% & 17,272 & 92.75\% \\ \hline
Connected & 4,767 & 2.11\% & 623 & 3.35\% \\ \hline
Intersecting & n/a & n/a & 727 & 3.90\% \\ \hline
\end{tabular}
\caption{Connectivity of regions in \DECO files}
\label{tab:connectivity}
\end{table}

In the following experiments, we use the detection of connected components as a reference baseline to compare the results of our more sophisticated approach involving element partitioning.

% As described in Section~\ref{subsec:clustering}, after recognizing candidate elements, our approach performs clustering based on a distance composed of three features: geometric distance, size ratio and alignment.
% These terms are calculated such that pairs of elements with lower score have higher probability of being grouped together.

% To validate our intuitions behind the design of these terms, we computed the scores for all the possible pairs of annotated elements in each DECO file, and compared the results of pairs of elements belonging to the same region (\emph{intra-region}) with those belonging to different regions (\emph{inter-region}).
% To avoid bias due to a different number of regions and elements in files, we take the average score of intra-region and inter-region pairs in a given file.
% Additionally, given the impact of file size on distances, we normalize the absolute values dividing them for file area.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figure/chap5/exp1/hyperparameters.png}
%     \caption{Distribution of inter- and intra-region distances}
%     \label{fig:distances}
% \end{figure}

% The results are showed in the box and whisker plot of Figure~\ref{fig:distances}: it can be noted how all three features have higher medians and averages for inter-region pairs, as well as overall more variance, with longer tailed distributions.
% The distributions of the first two features for intra-region element pairs are also significantly more concentrated around their medians, while the alignment difference show a wider spectrum of values.
% Overall, these qualities suggest that these features are appropriate in discriminating elements belonging together, even though some caution is needed while combining them together due to the different scales.

% The next subsection reports the results of the experiments conducted to find the optimal radius that guarantees best results for a given configuration of the three distance weights.

==> experiments/old/2_hyperparameters.tex <==
\subsection{Optimal hyperparameter selection}
\label{subsec:evaluation-radius}

As described in Section~\ref{subsec:region-detection}, the most important parameter to influence the performance of our clustering approach is the radius of the search space. 
Before reporting on the overall detection result, we analyze the effect of this parameter to guide an optimal choice.

The statistics that we present in this section are obtained running our clustering method on each file, varying the size of the radius in a grid with boundaries (0.1,10) and a spacing of~0.1.
The expected effect of the increase in radius size is the decrease in the number of the final clusters, as it allows more and more distant elements to be grouped together. 
We interrupted the radius progression in case the number of detected regions in a file reached~1.

Additionally, we experimented with different configurations of the distance features' weights.
We kept $\alpha=1$ as a fixed reference value and varied $\beta, \gamma \in \{0, 0.5, 1, 5, 10\}$.
We present the radius analysis for the hyperparameter configuration that showed the best results, which correspond to $\alpha=1, \beta=0.5, \gamma=1$.


Figure~\ref{fig:radii-distribution} shows the distribution of optimal radii across the dataset files.
Their majority is spread across lower values.
% TODO CHANGE RESULTS HERE
It is noteworthy how no file shows an optimal radius in the range $(0.5,1)$: a possible explanation is that values in this range are either not large enough for spreadsheets with widespread regions, or too large for those characterized by ``tightly knit'' regions.
As the chart shows, only a few files have an optimal radius above 5.0, demonstrating a sufficiently wide choice of the search grid boundaries.
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{figure/chap5/radius-distribution.png}
    \caption{Distribution of optimal radii}
    \label{fig:radii-distribution}
\end{figure}

Considering the discovered spectrum of possible optimal radii, the next experiment aimed at finding whether different properties of files correlate with their optimal radius.
% In particular, we are interested in discovering correlation between a-priori measurable quantities, to heuristically guide the choice of the radius for unseen files.
We look for correlations with at least 95\% confidence and therefore consider only results whose p-value is less than~0.05.

The properties chosen are the file size and the three distances that are on the basis of the clustering algorithm.  
They are calculated pair-wise on the set of connected components~(C) and partitioned elements~(P) for each file, and then averaged to obtain a single value to correlate with the optimal radius for the given file.
% In case a single file didn't contain two elements, or two partitions, we set the corresponding average measures to~0.
To compensate for the effect of file size on the average geometric distance of the elements, we also computed a correlation score normalizing the distance per file size.

Table~\ref{tab:radius-correlation} shows the results of the experiments.
The correlations outlined in bold, albeit weak, are the three highest found.
% For these, the p-values are lower than the specified 0.05 threshold, therefore we can consider them relevant.
% It is interesting to note how the average element distance appears relevant only after normalizing it by file size, showing the great influence of bigger files.
% Another trend can be seen analyzing how, 
In general, the connected component's features show a better correlation than those of the partitioned elements.
This proves how moving from a coarse-grained to a finer-grained element detection can cause loss of large-scale information.
Overall, the results of the analysis show a wide range of values for a tailored, ``dynamic'' choice of the radius.
Unfortunately, we were not able to find a strong correlation with any file property that could guide radius choice.

\begin{table}[ht]
%\def\arraystretch{1.5}
\centering
\begin{tabular}{l|r|l}
Measure (file-wise average) & Correlation & P-value \\ \hline
\multicolumn{1}{|l|}{File size } & -.0455 & \multicolumn{1}{l|}{.184} \\ \hline
\multicolumn{1}{|l|}{Distance (C)} & .1073 & \multicolumn{1}{l|}{.001} \\ \hline
\multicolumn{1}{|l|}{Distance (P)} & .0822 & \multicolumn{1}{l|}{.016} \\ \hline
\multicolumn{1}{|l|}{Distance, normalized (C)} & \textbf{.2516} & \multicolumn{1}{l|}{\boldmath{$9.05\cdot10^{-14}$}} \\ \hline
\multicolumn{1}{|l|}{Distance, normalized (P)} & \textbf{.1951} & \multicolumn{1}{l|}{\boldmath{$9.25\cdot10^{-9}$}} \\ \hline
\multicolumn{1}{|l|}{Alignment (C)} & .0300 & \multicolumn{1}{l|}{.380} \\ \hline
\multicolumn{1}{|l|}{Alignment (P)} & .1012 & \multicolumn{1}{l|}{.003} \\ \hline
\multicolumn{1}{|l|}{Size ratio (C)} & \textbf{.2479} & \multicolumn{1}{l|}{\boldmath{$2.09\cdot10^{-13}$}} \\ \hline
\multicolumn{1}{|l|}{Size ratio (P)} & .1246 & \multicolumn{1}{l|}{$2.63\cdot10^{-4}$} \\ \hline
\end{tabular}
\caption{Correlation between distances and optimal radius}
\label{tab:radius-correlation}
\end{table}

To avoid file-tailored hyperparameter selection, we also experimented to find the best ``static'' radius, i.e., the one with the most consistent results for all spreadsheets of the dataset.
For this, we fixed the hyperparameters $\alpha, \beta, \gamma$ with the best values found experimenting for the dynamic radius selection, i.e., 1, 0.5 and 1, respectively.
%TODO CHANGE PARAMETERS ?
Then we performed sampling in the interval $[0.1, 2.0]$, with a spacing of~0.1, and selected the one with the best performances on the dataset, namely~1.5.

==> experiments/old/4_binaryclassification.tex <==
\subsection{Multiregion classification}
\label{subsec:evaluation-binary}

The first task, which we refer to as \textit{\multifile~classification}, is the binary task of recognizing whether a given file contains one or multiple independent regions.
In other words, if a file is found to have more than one region, it is labeled as being ``\multifile'', and needs to be split into different pieces according to different region boundaries.
%To obtain a binary score, for every approach we consider the detected number of regions. In case of more than one region found, the file is labeled as being ``multitable''.
In comparing the results with the gold standard, we examine binary accuracy, precision, and recall.
Figure~\ref{fig:binary-classification} compares the results for the multitable classification task obtained by the different approaches.
\begin{figure}[ht]
    \centering
    % \includegraphics[width=\linewidth]{figure/chap5/binary_2.png}
    \includegraphics[width=\linewidth]{figure/chap5/binary_mondrian.png}
    \caption{Results on the binary classification task}
    \label{fig:binary-classification}
\end{figure}

The best results are obtained with our clustering approach and choosing an appropriate radius for each file.
With respect to radius choice, we labeled this setup as ``dynamic'', considering that for each file a different radius is chosen, as opposed to the ``static'' assignment of one, fit-for-all radius.
Because the ``dynamic'' results are obtained using knowledge of each file to select the best radius, they are to be considered an upper bound to illustrate the possibilities of our approach if the best parameters are selected.

The figure shows how both the clustering and the connected component approaches are satisfactory in detecting whether a file is multitable or not.
% Interestingly, the results from the static radius clustering are overlapping with those of the connected component detection.
% This suggests that the best choice for a static radius is a ``conservative'' value that can has the effect of degrading clustering to connected component detection.

On one hand, the connected component detection has better recall than the clustering with a static choice of the radius.
In fact, the single region files with only one connected component are always correctly classified, while the clustering approach could possibly partition connected components in finer-grained elements and lose recall.
This loss is traded off by higher precision since our approach is able to deal with adjacent and apparently separated tables.

The genetic-based approaches, regardless of the level of input features used, are not able to reach sufficiently good performances.
Their precision is high, but the recall is poor: this might be due to their focus on recognizing specific tabular structures, which leads to trying to forcibly fit regions into one table whenever they should be split.

%The results of this experiment show that we can positively answer the first research question posed in Section~\ref{subsec:problem}: it is possible, using our approach with correctly tuned parameters, to automatically recognize multitable files that need splitting.

% The next experiments will analyze the performances of the approaches in more depth, by evaluating region boundary detection.

==> experiments/old/6_files.tex <==
\subsection{File-wise accuracy}
\label{subsec:evaluation-gui}

\begin{figure*}[t]
\centering
% \includegraphics[width=0.8\linewidth]{figure/chap5/edit_distances_2.png}
\includegraphics[width=0.8\linewidth]{figure/chap5/edit_mondrian.png}
\caption{File-wise edit distances histogram and cumulative distribution.}
\label{fig:edit-distances}
\end{figure*}

The intended use-case of \systemname is to assist users in preparing \multifile~spreadsheet files.
Thus, we now analyze its usefulness by generating initial cluster candidates for the regions and then allowing users to correct the results as needed.
%As we have found out in the previous experiment, it is unrealistic to fully automatically split all regions with the results of any of the approaches under consideration.
%The focus of the next experiment is to evaluate how correct is the automatic region detection on a per-file basis and what is the margin of improvement using automated approaches over manual detection.
To do so, we designed an edit distance to reflect for each file the number of adjustments needed to match the predicted regions to the desired target.

We allow three operations: resizing an incorrect region, adding a new region and deleting an existing one.
These operations can also be linked with user interactions on our graphical interface (described in Section~\ref{subsec:gui}) to manually adjust the results of the automated table detection before file splitting.
We consider all three operations as equally expensive.
In the case of additions, a related resizing operation must be also carried out to obtain the desired shape and position of the region.

In Figure~\ref{fig:edit-distances} we report the distribution of edit costs on a file-wise basis: the $y$ coordinates of the bars correspond to the percentage of files in the dataset for which $x$ edits are needed on the detected regions to reach perfect boundaries.
The dashed lines plot the cumulative percentage of files covered as the number of edits increases.

The results show that when looking at single files, with a static radius choice, around a fourth of them can be correctly split according to the tables automatically detected -- the results need no edits.
Moreover, exploiting the results of our approach requires fewer corrections than any alternative for almost 70\% of the files.

For the remaining files, it seems that having no previous detection requires the same number or fewer user interactions than any other automated approach. 
In this scenario, the number of edits always corresponds to adding and resizing a new rectangle for each of the regions in the file and is directly proportional to the number of regions.
We can consider files with a greater number of necessary user interactions as ``hard'' to prepare using automated approaches.

The connected component detection has the highest fraction of such files.
This is consistent with the analysis of Tables~\ref{tab:average-regions} and~\ref{tab:connectivity} (Section~\ref{subsec:evaluation-dataset}), which reported the high average number of regions in multitable files (almost~11), and their un-connectedness.

The genetic-based approaches require more interventions than any other approach for most files to reach perfect results.
Considering the low percentages of detected regions and table boundaries, this outcome is not surprising.

Even though having a file-wise optimal radius yields a higher percentage of spreadsheets that need no edits, an interesting result is that clustering with a static radius still needs only a few corrections and actually proves to be better for hard files.

In the histogram, we can observe a characteristic behavior: a marginal number of files that need only one edit in the clustering case, as well generally more files requiring an odd number of edits.
The former is due to the nature of the approach: since all non-empty cells are part of a cluster, the minimum correction needed is almost always a resize plus an addition if two tables are incorrectly grouped, or a delete and a resize if one table is incorrectly split.
The only possibility of having one action is a resize for one of two tables intersecting each other.
The latter observation can also be explained with the same phenomenon: since most edits require pairs of actions, and the addition brings a necessary resize for the added region, there are higher chances of having an odd number actions, e.g., one addition and two resizes, or one delete, one addition, and three resizes.

Ultimately, the results proved that our clustering approach, with the hyperparameters provided ($r=1.5,\ \alpha=1,\ \beta=0.5,\ \gamma=1$), leads to reasonable region boundaries that can be exploited by users to split \multifile~spreadsheets with a significantly lower number of edits than any other previously existing region detection approach.

% To conclude the evaluation section, the last experiment gives an insight on the time complexity for our approach, with an analysis of its running times.

==> experiments/old/8_time.tex <==
\subsection{Execution time performance}
Our last experiment evaluates the time complexity of \systemname, analyzing the run-time from file loading to the output of the automated detection results.
The times were recorded on a consumer machine, equipped with a 6-core Intel i7-8750H CPU with a base frequency of 2.20GHz and 16GB of RAM, running the 64-bit version of the operating system Ubuntu 19.10 with the 5.3.0 version of the Linux kernel.
The code was written and executed using Python~3.7.5, limited to the use of nine cores out of the 12 available on the machine, to reproduce a non-exclusive usage scenario.

The tests were conducted in five independent runs: Figure~\ref{fig:runtime} presents the average run-time for each file.
The standard deviations of the times for each file did not indicate significant time variance across runs.
The plot shows the execution times against the area of the files, using a ``symmetrical logarithmic'' (symlog) scale, i.e.,  a linear scale in $[0,1]$ and a logarithmic scale in $[1,1000]$.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/chap5/time_performances.png}
    \caption{Mondrian run-times per files sorted by their area}
    % \caption{Clustering run-times per files sorted by their area}
    \label{fig:runtime}
\end{figure}

% Each point also has an associated error bar corresponding to the standard deviation of the observations.

Overall, more than 75\% of the spreadsheets are processed in under two seconds, which can be considered a satisfactory performance considering the interactive nature of the file splitting task.
Additionally, since the clustering scales with the number of atomic data regions identified, we observe good performances even in larger files, as suggested by the presence of vertical stripes on the left part of the scatter plot.
However, as it can be expected, a trend shows a weak correlation between higher time expense and more ``complicated'' files, with a handful of large outliers processed in more than one minute.


==> gui.tex <==
\subsection{User interface}
\label{subsec:gui}

We designed a web-based graphical interface to efficiently carry out \multifile~file splitting after regions are automatically detected.

Users are able to load a given spreadsheet file, run our \systemname algorithm, and visualize its results as rectangular overlays on the spreadsheet cells (Figure~\ref{fig:gui}).
With simple (and hopefully few) mouse interactions, the tool allows to adjust the size of the rectangles, drag and drop them along cells, as well as create or delete existing rectangles.
\begin{figure}[ht]
\centering
{\efbox{\includegraphics[width= 0.97\linewidth]{figure/chap4/gui.png}}}
\caption{Tool for interactive table splitting.}
\label{fig:gui}
\end{figure}

Once users are satisfied with number, shape, and position of the rectangles, they trigger a file split that will create a set of files, each containing the cells corresponding to one of the regions.
In Section~\ref{subsec:evaluation-gui} we evaluate the effort needed by users to correct the clustering results and reach intended results using the graphical interface provided.


==> stub.tex <==
% As an example, Figure~\ref{fig:overview} depicts the visual structure of three real spreadsheet files that contain three independent data regions with the same layout, inspiring us to name our approach after the abstract painter Piet Mondrian.
% As a real-world example of spreadsheets from the same layout template, consider the United States Census data, made publicly available through an open data portal.

% As an example, Figure~\ref{fig:overview} depicts the visual structure of a real spreadsheet file that contains three independent data regions, inspiring us to name our approach after the abstract painter Piet Mondrian.
% \begin{figure}[t]
% \centering
% \includegraphics[width=.6\columnwidth]{figure/chap1/segmentation.png}
% \caption{Visually splitting a complex \multifile~file.}
% \label{fig:overview}
% \end{figure}

% To process the data contained in different regions, a user is forced to split the file, after having recognized its arbitrary structure.
% What is more, it is usual for multiregion layouts to repeat similarly across different spreadsheet files, especially from the same source. 
% Equal structures repeating across different files constitute a ``layout template''. 

% All files of a template have the same number of regions, arranged in the same  positions, and even if the content of their data regions is different, they have equivalent metadata regions (for a more formal definition, cf.\ Section~\ref{subsec:recurring}).

% Our goal is to first identify different regions in single spreadsheets and describe their layout and then to find file \emph{templates}, i.e., classes of files showing the same region layout.
% to make them easier to analyze and prepare uniformly.
% Therefore, to achieve the most generality possible, we design our approach, \systemname, to exploit the literal content and visual distribution of cells in \multifile~files. 


==> taxonomy.tex <==
\subsection{Taxonomy of layouts}
\label{subsec:taxonomy}
In practice, the unconstrained nature of spreadsheet files leads to a plethora of possible layouts. We focus our attention on files that are not trivial to characterise, i.e., that contain a minimum of two elements.
We identify four primitive layouts, that can be further composed:
\begin{itemize}
\item \textbf{Apparently separated region}: A single region $R$ composed of more than one non-empty element is apparently separated if there exist at least one node in its graph for which its incident edges all have feature vectors with distance~$>0$.
% \[
% \exists\ e_i, e_j \in \mathcal{E}_{\setminus\textbf{empty}} \bigm|\ e_i,\ e_j\ \textit{are not connected}
% \]

\item \textbf{Separated regions}:
Two regions $R_1$ and $R_2$ are separated if the feature vector of their relationship has a distance~$>0$.

\item \textbf{Adjacent regions}:
Two regions $R_1$ and $R_2$ are adjacent if the feature vector of their relationship has an $H$ or $V$ alignment direction with a magnitude~$>0$ and a distance~$=0$.

% at least two elements from the two respective regions are connected:
% \[
% \exists\ e^1_i \in \mathcal{E}_1, e^2_j \in \mathcal{E}_2\ \bigm|\ e^1_i,\ e^2_j\ \textit{are connected}
% \]

\item \textbf{Overlapping regions}:
Two regions $R_1$ and $R_2$ are overlapping if the feature vector of their relationship has an alignment direction of $O$ (overlapping) with a magnitude~$>0$.

% the bounding rectangles for the element sets $\mathcal{E}_1, \mathcal{E}_2\ $ are overlapping.
\end{itemize}

Figure~\ref{fig:taxonomy} shows real-wold examples from the DECO dataset (Cf.\ Section~\ref{sec:relatedwork}) for each one of these primitive layouts.

\begin{figure}[ht!]
% \hspace*{\fill}
\subcaptionbox{An apparently separated region\label{fig:tax-a}.}[\linewidth]
{\includegraphics[width=0.8\linewidth]{figure/chap3/apparent_mark.png}}
\subcaptionbox{Two separated regions\label{fig:tax-b}.}[\linewidth]
{\includegraphics[width=0.8\linewidth]{figure/chap3/separated_mark.png}}
\subcaptionbox{Two adjacent regions. \label{fig:tax-c}}[\linewidth]
{\includegraphics[width=0.8\linewidth]{figure/chap3/adjacent_mark.png}}
\subcaptionbox{Two overlapping regions.
\label{fig:tax-d}}[\linewidth]
{\includegraphics[width=0.8\linewidth]{figure/chap3/intersecting.png}}
\caption{Region layouts and their graph representations.}
\label{fig:taxonomy}
\end{figure}
